Rendering Participating Media Using Path Graphs

Rendering volumetric scattering media, including clouds, fog, smoke, and other complex materials, is crucial for realism in computer graphics. Traditional path tracing, while unbiased, requires many long path samples to converge in scenes with scattering media, and a lot of work is wasted by paths that make a negligible contribution to the image. Methods to make better use of the information learned during path tracing range from photon mapping to radiance caching, but struggle to support the full range of heterogeneous scattering media. This paper introduces a new volumetric rendering algorithm that extends and adapts the previous \emph{path graph} surface rendering algorithm. Our method leverages the information collected through multiple-scattering transport paths to compute lower-noise estimates, increasing computational efficiency by reducing the required sample count. Our key contributions include an extended path graph for participating media and new aggregation and propagation operators for efficient path reuse in volumes. Compared to previous methods, our approach significantly boosts convergence in scenes with challenging volumetric light transport, including heterogeneous media with high scattering albedos and dense, forward-scattering translucent materials, under complex lighting conditions.

==> macros_source.tex <==
%!TEX root = paper.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Additional packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% extra options for table
% remove this if thing looks different
\usepackage{colortbl}
\usepackage{xcolor}
\usepackage{xfrac}
\usepackage{float}
\usepackage{booktabs} % For formal tables
\usepackage{rotating}
\usepackage{paralist}
\usepackage{url}
%\usepackage[usenames,dvipsnames]{xcolor}
% \hypersetup{
%   colorlinks=true,
%   linkcolor=black,
%   citecolor=black,
%   urlcolor=black,
%   breaklinks=true,
%   draft=true       % set to true if you get errors about a link spanning page breaks
% }
% \hypersetup{draft}  % uncomment if you get errors about a link spanning page breaks
\usepackage{amsmath,amssymb,bm}
\usepackage{mathtools}
% \usepackage{pdfpages}
\usepackage{graphicx,wrapfig}
\usepackage{adjustbox}
\usepackage{subfig}
\usepackage{units}
\usepackage{soul}
\usepackage{calc}
\usepackage{tikz}
\usepackage{xspace}
\usepackage{microtype}
\usepackage[percent]{overpic}
\usepackage{enumitem}
\usepackage{afterpage}
\usepackage[normalem]{ulem}  % for strike-through (\sout)
\usepackage{multirow}
\usepackage{siunitx}
\usepackage{physics}
\usepackage{geometry}
\usepackage[makeroom]{cancel}
\usepackage{bm}
%\usepackage{titlesec}
\usepackage[utf8]{inputenc}
% for commenting
%\usepackage[draft]{pdfcomment}  % for work in progress
\usepackage[final]{pdfcomment}  % for Final draft
\usepackage[outline]{contour}
\contourlength{0.1em}%
\usepackage{tcolorbox}
\usepackage[percent]{overpic}
\usepackage{contour}

%Comments
% Select the type of commenting you want to use: none, pdf margin comments, or in-text comments
% \newcommand{\COMMENT}[3]{}  % for Final draft, removes comments
% \newcommand{\COMMENT}[3]{\pdfcomment[avatar=#1]{#1: #3}}  % For work in progress using PDF annotations
\newcommand{\COMMENT}[3]{\textcolor{#2}{{\footnotesize[\textsc{#1}: #3}]}}  % For work in progress using in-text comments

%\titlespacing*{\paragraph}{0pt}{0.2\baselineskip}{\baselineskip}

\newcommand{\TODO}[1]{\COMMENT{TODO}{red}{#1}}
\newcommand{\XD}[1]{\COMMENT{XD}{teal}{#1}}
\newcommand{\HB}[1]{\COMMENT{SJ}{blue}{#1}}
\newcommand{\IGNORE}[1]{}

\definecolor{DarkGreen}{rgb}{0.0,0.6,0.2}
% \newcommand{\REMOVE}[1]{{\color{red}\sout{#1}}} % for work in progress
% \newcommand{\ADD}[1]{{\textcolor{DarkGreen}{#1}}} % for work in progress    we
\newcommand{\REMOVE}[1]{} % for final version
\newcommand{\ADD}[1]{#1} % for final version
\newcommand{\REPLACE}[2]{\ADD{#2}} % for work in progress, showing the old text


\definecolor{CancelColor}{rgb}{0.7,0.7,0.7}
\renewcommand{\CancelColor}{\color{CancelColor}}

%References
\def\figureautorefname{Fig.}
\def\tableautorefname{Table}
\def\partautorefname{Part}
\def\sectionautorefname{Sec.}
\def\subsectionautorefname{Sec.}
\def\subsubsectionautorefname{Sec.}
\def\appendixautorefname{Appendix}
% Wrap equation numbers in parenthesis when using autoref, like eqref
\def\equationautorefname~#1\null{%
  Eq.~(#1)\null
}

\definecolor{camera-blue}{HTML}{1B75BB}
\definecolor{photon-orange}{HTML}{F79844}

%%Math
\def\approxprop{%
  \def\p{%
    \setbox0=\vbox{\hbox{$\propto$}}%
    \ht0=0.6ex \box0 }%
  \def\s{%
    \vbox{\hbox{$\sim$}}%
  }%
  \mathrel{\raisebox{0.7ex}{%
      \mbox{$\underset{\s}{\p}$}%
    }}%
}
\newcommand\Dirac{\delta}
\newcommand\Exp[1]{e^{#1}}
\newcommand{\dif}{\mathrm{d}}


\newcommand{\Paragraph}[1]{\subsubsection*{#1}}



% Light transport
\newcommand{\Point}{\mathbf{x}}
\newcommand{\Dir}{\vec{\mathbf{w}}}
\newcommand{\Dist}{w}
\newcommand{\Radiance}{L}
%\newcommand{\RadianceIn}[2]{\Radiance(#1\!\leftarrow\!#2)}
%\newcommand{\RadianceOut}[2]{\Radiance(#1\!\rightarrow\!#2)}
%\newcommand{\RadianceMedium}[2]{\Radiance_m(#1\!\leftarrow\!#2)}
%\newcommand{\Transmittance}[2]{T_r(#1 \leftrightarrow #2)}
\newcommand{\RadianceIn}[2]{\Radiance_i(#1,#2)}
\newcommand{\RadianceOut}[2]{\Radiance_o(#1,-#2)}
\newcommand{\RadianceMedium}[2]{\Radiance_m(#1,#2)}
\newcommand{\Transmittance}[1]{T_r(#1)}
\newcommand{\CoeffScatter}{\sigma_s}
\newcommand{\CoeffAbsorb}{\sigma_a}
\newcommand{\CoeffExtinct}{\sigma_t}
\newcommand{\Phase}[2]{f(#1 \cdot #2)}
\newcommand{\Normal}{\vec{\mathbf{n}}}
%
% Photon mapping
\newcommand{\Kernel}{K}
\newcommand{\Photon}{p}
\newcommand{\DirA}{\vec{\mathbf{a}}}
\newcommand{\DirB}{\vec{\mathbf{b}}}
\newcommand{\DirC}{\vec{\mathbf{c}}}
\newcommand{\DistA}{a}
\newcommand{\DistB}{b}
\newcommand{\DistC}{c}
\newcommand{\Width}{u}
\newcommand{\Height}{v}
\newcommand{\Depth}{w}
\newcommand{\sBlurAxis}{\vec{\Width}}

\newcommand{\Power}{\Phi}
\newcommand{\QueryRegion}{R}

%Domains
\newcommand{\Sphere}{{S^2}}%

% Wojtek's new notation
\newcommand{\sSensor}{{W_\mathrm{e}}} % sensor sensitivity (emitted importance)
\newcommand{\sEmission}{{L_\mathrm{e}}} % emitted radiance

\newcommand{\sRadiance}{\ensuremath{L}\xspace}
\newcommand{\sPos}{\ensuremath{\mathbf{x}}\xspace}
\newcommand{\sDir}{\ensuremath{\omega}\xspace}
\newcommand{\sDist}{\ensuremath{t}\xspace}
\newcommand{\sMergingIndex}{\ensuremath{1}\xspace}
\newcommand{\sLastLPathIndex}{\ensuremath{l}\xspace}
\newcommand{\sLastCPathIndex}{\ensuremath{k}\xspace}
\newcommand{\sPosPath}{\ensuremath{\overline{\sPos}}\xspace}
\newcommand{\sDirPath}{\ensuremath{\overline{\sDir}}\xspace}
\newcommand{\sDistPath}{\ensuremath{\overline{\sDist}}\xspace}
\newcommand{\sPosSubPath}[2]{\ensuremath{\sPos_{#1} \ldots \sPos_{#2}}}
\newcommand{\sDirSubPath}[2]{\ensuremath{\sDir_{#1} \ldots \sDir_{#2}}}
\newcommand{\sDistSubPath}[2]{\ensuremath{\sDist_{#1} \ldots \sDist_{#2}}}


\newcommand{\sCPos}{\ensuremath{\mathbf{y}}\xspace}
\newcommand{\sCDir}{\ensuremath{\psi}\xspace}
\newcommand{\sCDist}{\ensuremath{s}\xspace}
\newcommand{\sCMergingIndex}{\ensuremath{1}\xspace}
\newcommand{\sCPosPath}{\ensuremath{\overline{\sCPos}}\xspace}
\newcommand{\sCDirPath}{\ensuremath{\overline{\sCDir}}\xspace}
\newcommand{\sCDistPath}{\ensuremath{\overline{\sCDist}}\xspace}
\newcommand{\sCPosSubPath}[2]{\ensuremath{\sCPos_{#1} \ldots \sCPos_{#2}}}
\newcommand{\sCDirSubPath}[2]{\ensuremath{\sCDir_{#1} \ldots \sCDir_{#2}}}
\newcommand{\sCDistSubPath}[2]{\ensuremath{\sCDist_{#1} \ldots \sCDist_{#2}}}

\newcommand{\sFPos}{\ensuremath{\mathbf{z}}\xspace}
\newcommand{\sFPosPath}{\ensuremath{\overline{\sFPos}}\xspace}
\newcommand{\sFPathDomain}{\ensuremath{\Omega}}

\newcommand{\sMeasurement}{\ensuremath{I}}


% \newcommand{\sMeasure}[1]{\ensuremath{\mu(#1)}}
\newcommand{\sMeasure}{\ensuremath{\mu}}

\newcommand{\la}{\!\leftarrow\!}
\newcommand{\ra}{\!\rightarrow\!}
\newcommand{\lra}{\!\leftrightarrow\!}

\newcommand{\sVisibility}{\ensuremath{V}}
\newcommand{\sVisibilityFunc}[1]{\ensuremath{\sVisibility(#1)}}
\newcommand{\sTrans}{{\ensuremath{T_{\mathrm{r}}}}}
\newcommand{\sTransFunc}[1]{\ensuremath{\sTrans(#1)}}

\newcommand{\sExtinctionCoeff}{\sigma_t}
\newcommand{\sAbsorptionCoeff}{\sigma_a}
\newcommand{\sScatteringCoeff}{\sigma_s}

\newcommand{\sThroughput}{f}             % (sub)path throughput
\newcommand{\sWeight}{C}
\newcommand{\sWeightDensity}{\langle D \rangle}
\newcommand{\sPdf}{\ensuremath{p}\xspace}
\newcommand{\sScattering}{\rho}
\newcommand{\sBRDF}{\sScattering_\mathrm{s}} % BSDF
\newcommand{\sPhase}{\sScattering_\mathrm{p}} % phase function
\newcommand{\sMergeScattering}{\sThroughput_\sDir^{\sMergingIndex,\sCMergingIndex}}

\newcommand{\sBoundsMin}{\sCDist_{\sCMergingIndex-}}
\newcommand{\sBoundsMax}{\sCDist_{\sCMergingIndex+}}

\newcommand{\tracklength}[1]{\Delta #1}
\newcommand{\sEst}[1]{\langle #1 \rangle}
\newcommand{\sIntegralTrans}{\hat{\sTrans}}
\newcommand{\sIntegralTransSquared}{\hat{\sTrans^2}}
\newcommand{\abstractEstSymbol}{A}
\newcommand{\abstractEst}{\sEst{\abstractEstSymbol}}
\newcommand{\abstractEstFunc}[1]{\sEst{\abstractEstSymbol(#1)}}
\newcommand{\collisionEstSymbol}{C}
\newcommand{\tracklengthEstSymbol}{T}
\newcommand{\expectedEstSymbol}{E}
\newcommand{\transEst}[1]{\sEst{\sTrans}_#1}
\newcommand{\transEstFunc}[2]{\sEst{\sTrans(#2)}_#1}
\newcommand{\intTransEst}[1]{\sEst{\sIntegralTrans}_#1}
\newcommand{\intTransEstFunc}[2]{\sEst{\sIntegralTrans(#2)}_#1}
\newcommand{\collisionEst}{\intTransEst{\collisionEstSymbol}}
\newcommand{\tracklengthEst}{\transEst{\tracklengthEstSymbol}}
\newcommand{\expectedEst}{\transEst{\expectedEstSymbol}}
\newcommand{\collisionEstFunc}[1]{\intTransEstFunc{\collisionEstSymbol}{#1}}
\newcommand{\tracklengthEstFunc}[1]{\transEstFunc{\tracklengthEstSymbol}{#1}}
\newcommand{\expectedEstFunc}[1]{\transEstFunc{\expectedEstSymbol}{#1}}

\newcommand{\sKernel}{K}
\newcommand{\Dep}[1]{\tilde{#1}}


\let\oldabs\abs % Store original \abs as \oldabs
\let\abs\undefined % "Undefine" \abs
\DeclarePairedDelimiter\abs{\lvert}{\rvert}


% Xi Deng's notation
\newcommand{\sDistFunc}[1]{\ensuremath{{\sThroughput}_{\sDist}(#1)}}
\newcommand{\sDirFunc}[1]{\ensuremath{{\sThroughput}_{\sDir}(#1)}}
\newcommand{\sPdfArea}[1]{\ensuremath{{p_A}(#1)}}
\newcommand{\sPdfDist}[1]{\ensuremath{{p_t}(#1)}}
\newcommand{\sPdfDir}[1]{\ensuremath{{p_{\sDir}}(#1)}}
\newcommand{\sPdfLDir}[1]{\ensuremath{{p_L}(#1)}}
\newcommand{\sPdfSDir}[1]{\ensuremath{{p_S}(#1)}}
\newcommand{\sSampleDistTerm}[1]{\ensuremath{R_\sDist(#1)}}
\newcommand{\sSampleDirTerm}[1]{\ensuremath{R_\sDir(#1)}}
\newcommand{\sSampleEmTerm }{\ensuremath{R_e}}
\newcommand{\sPathWeight}{\ensuremath{R}}

\newcommand{\Root}{*}

\newcommand{\sVar}{\ensuremath{\xi}}
\newcommand{\sVarParam}[2]{\xi_{#1}^{#2}}
\newcommand{\sVarSetParam}[2]{\ensuremath{\overline{\sVar_{#1}^{#2}}}}
\newcommand{\sVarSet}{\sVarSetParam{}{}}
\newcommand{\sAVarSet}{\sVarSetParam{a}{}}
\newcommand{\sNVarSet}{\sVarSetParam{n}{}}
\newcommand{\sAVarSetRoot}[1]{\sVarSetParam{a}{\Root#1}}


% \newcommand{\Kernel}[1]{\bm{\delta}_{#1}}
\newcommand{\Jacob}[2]{\mathbf{J}_{#1}^{#2}}
\newcommand{\DenEst}[1]{\mathbf{D}_{#1}}

\newcommand{\TKernel}[1]{\ensuremath{\delta^3(#1)}} %Three dimension kernel
\newcommand{\SKernel}[1]{\ensuremath{\delta^2(#1)}} %Two dimension kernel
\newcommand{\OKernel}[1]{\ensuremath{\delta(#1)}} %One dimension kernel

% parameter spaces
\newcommand{\Amatrix}{\mathbf{A}}
\newcommand{\Zero}{\mathbf{0}}
\newcommand{\tts}{\sDist_2, \sDist_1, \sCDist_1}
\newcommand{\uts}{u, \sDist_l, \sCDist_1}
\newcommand{\vts}{v, \sDist_l, \sCDist_1}
\newcommand{\uvs}{u, v, \sCDist_1}
\newcommand{\xyz}{x, y, z}
\newcommand{\upts}{u', \sDist_1, \sCDist_1}
\newcommand{\vpts}{v', \sDist_1, \sCDist_1}

% Vectors and points
\newcommand{\Uax}[1]{\mathnormal{u}(#1)}
\newcommand{\Vax}[1]{\mathnormal{v}(#1)}
\newcommand{\OPoint}{\mathbf{o}}
\newcommand{\Uvec}{\mathbf{u}}
\newcommand{\Vvec}{\mathbf{v}}
\newcommand{\Vr}{\mathbf{r}}
\newcommand{\OPointP}{\mathbf{o'}}
\newcommand{\UvecP}{\mathbf{u_\bold{\alpha}}}
\newcommand{\Ua}{u_{\alpha}}
\newcommand{\VvecP}{\mathbf{v_\bold{\alpha}}}
\newcommand{\Center}{\mathbf{o_c}}
\newcommand{\PixIntensity}{\ensuremath{I}}
\newcommand{\sMisWeight}{\mathnormal{W}}
\newcommand{\Ivec}{\ensuremath{\vec{\mathbf{i}}}}
\newcommand{\Jvec}{\ensuremath{\vec{\mathbf{j}}}}
\newcommand{\Kvec}{\ensuremath{\vec{\mathbf{k}}}}
\newcommand{\Mnormal}{\ensuremath{\mathbf{n}}}


\newcommand{\Gf}{\mathbf{g}}


\newcommand{\Expect}[1]{\mathbb{E}[#1]}

\newcommand{\sFPathLength}{\mathnormal{h}}
\newcommand{\sPathLength}{\mathnormal{l}}
\newcommand{\sCPathLength}{\mathnormal{k}}
\newcommand{\sPScore}{\ensuremath{\mathnormal{s}}}
\newcommand{\sSampleAmount}{\ensuremath{{\mathnormal{n}}}}


\newcommand{\sMeasureVertex}{\ensuremath{\mu}}
% \newcommand{\sMeasureDD}{\ensuremath{\mu^{'}}}
% \newcommand{\sMeasureStandard}{\ensuremath{\mu^{*}}}

%space
\newcommand{\sTwoDSpace}{\ensuremath{\mathnormal{D}}}
\newcommand{\paraSpace}{\Xi}
\newcommand{\sExtendSpace}{\Omega}
\newcommand{\sStandSpace}{\Omega*}


% LaTeX does not allow numbers in macro identifiers, so
% III -> 3D blur, II -> 2D blur, etc.
% P -> point, B -> beam, Q -> quad (plane), C -> cube (parallelepiped)
\newcommand{\sPPIII}{\text{P-P3D}\xspace}
\newcommand{\sBPII}{\text{P-B2D}\xspace}
\newcommand{\sBBI}{\text{B-B1D}\xspace}
\newcommand{\sBBII}{\text{B-B2D}\xspace}
\newcommand{\sBQI}{\text{Q-B1D}\xspace}
\newcommand{\sBQ}{\text{Q-B0D}\xspace}
\newcommand{\sBC}{\text{C-B0D}\xspace}

%Contribution Function
\newcommand{\sContriV}{\ensuremath{f}}
\newcommand{\sContriD}{\ensuremath{f}}
\newcommand{\sGeoTerm}[1]{\ensuremath{G}(#1)}


% Captions
\newcommand{\bathroom}{Bathroom}
\newcommand{\bedroom}{Bedroom}
\newcommand{\kitchen}{Kitchen}
\newcommand{\livingroomtwo}{Living Room}
\newcommand{\livingroomthree}{Red Room}
\newcommand{\staircase}{Doorway}
\newcommand{\staircasetwo}{Staircase}


%\newcommand{\inlineOrFigure}[2]{#2}
\newcommand{\inlineOrFigure}[2]{#1}

\newcommand{\KernelWidth}{\Width}



%SJ's macros
\newcommand{\I}{_i}
\newcommand{\II}{_j}
\newcommand{\III}{_k}
\newcommand{\isol}{_r}
\newcommand{\solm}{^{*_r}}
\newcommand{\sumsol}{\sum\isol}

\newcommand{\reffig}[1]
{
Fig.\ref{fig:#1}
}

\newcommand{\reftab}[1]
{
Table.\ref{#1}
}

\newcommand{\refeqt}[1]
{
Eq.\ref{#1}
}

\newcommand{\pd}[2]
{
\frac{\partial #1}{\partial #2}
}

\newcommand{\pdt}[2]
{
\nicefrac{\partial #1}{\partial #2}
}


\newcommand{\proot}[1]
{
\sPos_{#1}^\Root
}

\newcommand{\droot}[1]
{
\sDir_{#1}^\Root
}

\newcommand{\phiroot}[1]
{
\phi_{#1}^\Root
}

\newcommand{\costhetaroot}[1]
{
\cos{\theta}_{#1}^\Root
}


\newcommand{\troot}[1]
{
\sDist_{#1}^\Root
}

\newcommand{\ctheta}[0]
{
\cos{\theta}
}

\definecolor{darkgreen}{rgb}{0.05,0.6,0.05}


\usepackage{pbox}
\usepackage{booktabs}
% \usepackage{graphicx}



% some lengths that are used for tikzpicture figures
\newlength{\mygrid}%
\newlength{\myimg}%
